Dealing with quantum computer readout noise through high energy physics unfolding methods

Quantum computers have the potential to solve problems that are intractable to classical computers, nevertheless they have high error rates. One significant kind of errors is known as Readout Errors. Current methods, as the matrix inversion and least-squares, are used to unfold (correct) readout errors. But these methods present many problems like oscillatory behavior and unphysical outcomes. In 2020 Benjamin Nachman et al. suggested a technique currently used in HEP, to correct detector effects. This method is known as the Iterative Bayesian Unfolding (IBU), and they have proven its effectiveness in mitigating readout errors, avoiding problems of the mentioned methods. Therefore, the main objective of our thesis is to mitigate readout noise of quantum computers, using this powerful unfolding method. For this purpose we generated a uniform distribution in the Yorktown IBM Q Machine, for 5 Qubits, in order to unfold it by IBU after being distorted by noise. Then we repeated the same experiment with a Gaussian distribution. Very satisfactory results and consistent with those of B. Nachman et al., were obtained. After that, we took a second purpose to explore unfolding in a larger qubit system, where we succeed to unfold a uniform distribution for 7 Qubits, distorted by noise from the Melbourne IBM Q Machine. In this case, the IBU method showed much better results than other techniques.

==> Chapters/Abbreviations/abbreviations.tex <==
% First parameter can be changed eg to "Glossary" or something.
% Second parameter is the max length of bold terms.
\begin{mclistof}{List of Abbreviations}{3.2cm}

\item[QC] quantum computer/quantum computing.

\item[R\&D] research and development.

\item[RCS] random circuit sampling.

\end{mclistof} 


==> Chapters/Abstract/abstract.tex <==
\begin{center}
\Huge\textsc{Abstract}
\end{center}

A quantum computer has the potential to solve problems that are intractable to classical computers, nevertheless they have high error rates. One significant kind of errors is known as “\textit{Readout Errors}”. Current methods are used to unfold (correct) these errors, as the \textit{matrix inversion} and \textit{least-squares} method. But They present several problems.

In 2020 \textsc{Benjamin Nachman} et al suggested a technique currently used in HEP, to correct detector effects. This method is known as the “\textit{Iterative Bayesian Unfolding}” (IBU), and they have proven its effectiveness in mitigating readout errors, avoiding problems of the mentioned methods.

Therefore, the main objective of our thesis is to mitigate readout noise of quantum computers, using this powerful unfolding method. For this purpose we generated a \textit{uniform distribution} in the \textsc{Yorktown IBM Q Machine}, for 5 Qubits, in order to unfold it by IBU, after its \textit{distortion} by noise, then we repeated the same experiment with a \textit{Gaussian distribution}, and very satisfactory results have been obtained, and which are consistent with those obtained by \textsc{B. Nachman} et al. After that, we took a $2^{nd}$ purpose to explore unfolding in a larger qubit system, where we unfolded a \textit{ uniform distribution} of 7 Qubits, distorted by the \textsc{Melbourne IBM Q Machine} noise, where the IBU showed much better results than other techniques.


==> Preamble.tex <==
\setlength{\textbaselineskip}{25pt plus3pt}
\setlength{\frontmatterbaselineskip}{20pt plus2pt minus1pt}
\setlength{\baselineskip}{\textbaselineskip}

\setcounter{secnumdepth}{3}
\setcounter{tocdepth}{4}
\usepackage{titlesec}
\usepackage{setspace}

\titleformat{\section}
{\color{blue!70!black}\normalfont\Large\bfseries}
{\color{blue!70!black}\thesection}{1em}{}



\usepackage[style=numeric-comp, sorting=none, backend=biber, doi=true, isbn=false]{biblatex}
\newcommand*{\bibtitle}{References}

\usepackage{lipsum}


\addbibresource{References.bib}



\usepackage{afterpage}

\newcommand\blankpage{%
    \null
    \thispagestyle{empty}%
    \addtocounter{page}{-1}%
	\newpage}
\usepackage{sidecap}
\setlength{\baselineskip}{25pt} 



	\renewcommand{\th}{\textsuperscript{th}} 
	\newcommand{\nd}{\textsuperscript{nd}}
	\renewcommand{\st}{\textsuperscript{st}}
	\newcommand{\rd}{\textsuperscript{rd}}


\usepackage[most]{tcolorbox}

\usepackage{titlesec}

\usepackage{wrapfig}
\usepackage{booktabs}
\usepackage[bottom]{footmisc}
%\renewcommand{\arraystretch}{1.7}
\usepackage{physics}
\usepackage{caption}
\usepackage{mwe}
\usepackage{float}
\usepackage{marginnote}
\usepackage{caption}
\SetLipsumParListSurrounders{\colorlet{oldcolor}{.}\color{gray}}{\color{oldcolor}}
\usepackage{sidenotes}
%\usepackage[pdftex]{graphicx}

\usepackage[T1]{fontenc}

%\usepackage[table,xcdraw]{xcolor}

%\usepackage{floatrow}

\usepackage[T1]{fontenc}
\usepackage[font=small,labelfont=bf,tableposition=top]{caption}

\usepackage[utf8]{inputenc}
\usepackage{babel}
%\usepackage[font=small,labelfont=bf]{caption}



%\usepackage{capt-of}% or \usepackage{caption}
\usepackage{booktabs}
\usepackage{varwidth}
\newsavebox\tmpbox


\usepackage{qcircuit}

%\usepackage{tikz}
%\usetikzlibrary{quantikz}

\usepackage[define-L-C-R]{nicematrix}
\usepackage{amsmath}

%\usepackage{svg}
%%%%%%%%%%%%% Mise en page %%%%%%%%%%%%
\voffset=-0.04cm
\parindent=1cm
\raggedbottom
\abovedisplayskip=3mm
\belowdisplayskip=3mm
\abovedisplayshortskip=0mm
\belowdisplayshortskip=2mm
%\setlength{\parskip}{0.1cm}
%\setlength{\parindent}{1cm}
%%% suite %%%
%\setlength{\topmargin}{0cm} 
%\setlength{\topmargin}{0cm} 
%\setlength{\oddsidemargin}{0cm}
%\setlength{\evensidemargin}{0cm} 
\setlength{\textheight}{24.8cm}
\setlength{\textwidth}{17.0cm}
\hoffset=0cm
%%%%%%%%%% Fin de mise en page %%%%%%%%

%\theoremstyle{definition}
%\newtheorem{definition}{Definition}[section]
\newtheorem{definition}{Definition}[section]    %% this does it

%\theoremstyle{remark}
%\newtheorem*{remark}{Remark}

\usepackage{amsthm}
\setlength\parindent{0.5cm}
%**********************************************

\usepackage{cleveref}
\usepackage[most]{tcolorbox}

\newtcbtheorem[number within=chapter]{Theorem}{}{
        enhanced,
        sharp corners,
        attach boxed title to top left={
            xshift=-1mm,
            yshift=-5mm,
            yshifttext=-1mm
        },
        top=1.5em,
        colback=white,
        colframe=blue!75!black,
        fonttitle=\bfseries,
        boxed title style={
            sharp corners,
            size=small,
            colback=blue!75!black,
            colframe=blue!75!black,
        } 
    }{thm}

\newtcbtheorem[number within=chapter]{Definition}{}{
        enhanced,
        sharp corners,
        attach boxed title to top left={
            xshift=-1mm,
            yshift=-5mm,
            yshifttext=-1mm
        },
        top=1.5em,
        colback=white,
        colframe=blue!20!black,
        fonttitle=\bfseries,
        boxed title style={
            sharp corners,
            size=small,
            colback=blue!20!black,
            colframe=blue!20!black,
        } 
    }{def}

\newenvironment{myTheorem}[2]{ \begin{Theorem}[adjusted title=#1]{}{#2} 
  \textbf{Theorem \thetcbcounter.} }{\end{Theorem}}

  \newenvironment{myDefinition}[2]{ \begin{Definition}[adjusted title=#1]{}{#2} 
  \textbf{Definition \thetcbcounter.} }{\end{Definition}}
  
  \usepackage{sidecap}

\usepackage{mathtools,amssymb,amsthm}

\usepackage{minted}
%\usepackage{xcolor}

\definecolor{LightGray}{gray}{0.9}
%\definecolor{DarkGray}{gray}{0.1}

%\pagecolor{DarkGray}

\usemintedstyle{borland}

%New colors defined below
\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}


%SORTING LIST %%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{datatool}% http://ctan.org/pkg/datatool
\newcommand{\sortitem}[1]{%
  \DTLnewrow{list}% Create a new entry
  \DTLnewdbentry{list}{description}{#1}% Add entry as description
}
\newenvironment{sortedlist}{%
  \DTLifdbexists{list}{\DTLcleardb{list}}{\DTLnewdb{list}}% Create new/discard old list
}{%
  \DTLsort{description}{list}% Sort list
  \begin{itemize}%
    \DTLforeach*{list}{\theDesc=description}{%
      \item \theDesc}% Print each item
  \end{itemize}%
}

\usepackage{xcolor}
%\usepackage{listings}
\usepackage{minted}
\usemintedstyle{pastie}
\usepackage{xparse}

%%%\NewDocumentCommand{\codeword}{v}{%
%%%%\texttt{\textcolor{blue}{#1}}%
%%}
%%\lstset{language=Python,keywordstyle={\bfseries \color{blue}}}

\usepackage{minted}
\usepackage{lipsum}  
%%%\usepackage{listings}

\newminted{python}{fontsize=\small, 
                   linenos,
                   numbersep=8pt,
                   gobble=0,
                   breaklines,
                   frame=lines,
                   bgcolor=bg,
                   framesep=3mm} 
                   
\usepackage{mathtools,amssymb,amsthm}
\usepackage{physics}
\usepackage{graphicx}
\definecolor{bg}{rgb}{0.97,0.97,0.97}


